Towards a Platform for Mastering Personal Sovereignty

The ongoing digital transformation of work, administration, health, mobility, and social interaction is profoundly reshaping everyday life, steadily shifting control from individuals to large platform providers. Although data is often labeled the "gold of the 21st century", its real value is realized through services that access, combine, and exploit it. Today, individuals have little sovereignty: life events (e.g., changing an address, insurance, job, or marital status) require fragmented, repetitive interactions across numerous systems, leaving users overwhelmed rather than empowered. We argue for a fundamental rethinking of this situation and propose a virtual, trustworthy platform, called "MyVirtualME" that acts on behalf of the human individual towards companies, administrations, and other actors. This platform centers services, data, permissions, and data usage around humans, not foreign actors, allowing genuine control and transparency. Our vision goes beyond a pure data focus: supported by trusted services ranging from basic notifications to intelligent assistants, MyVirtualME aims to reduce digital bureaucracy, improve and even automate interactions, and support informed oversight of an individual's health, financial, and administrative situation. We firmly believe that a human-centered MyVirtualME is essential for restoring personal sovereignty in our digital future.

==> src/tex/inc/Listings.tex <==
%% listings
\usepackage{listings}
\lstset{
    numbers=left,
    numberstyle=\tiny,
    numbersep=5pt,
    frame=single,
    aboveskip=0pt,
    belowskip=0pt,
    sensitive=true,
    float=!t,
    breaklines=true,
    captionpos=b,
    tabsize=2,
    showstringspaces=false,
    basicstyle=\ttfamily\footnotesize, %basicstyle=\small\ttfamily,
    literate=
        {//WARNING}{{\includegraphics[width=8pt,height=8pt]{pic/warning.png}}}{2}
        {//ERROR}  {{\includegraphics[width=8pt,height=8pt]{pic/error.png}}}{2},
    morecomment=[l]{//}, 
    morecomment=[s][\itshape]{/**}{*/}
}

% % #1 language
% % #2 flag
% % #3 label
% % #4 caption
% % #5 file
% \newcommand{\lstinputSeparatedFlag}[5] {
%     \begin{ownfigure}
%     \vspace{2.5ex}
%     \setlength{\parskip}{1ex plus0pt minus0pt}\noindent%
%     \smash{\rlap{\hspace{0.75ex}\raisebox{-0.0ex}{\rightline{\scriptsize
%     \tt \frame{\makebox(80, 11){#2}}}}}}%
%     \lstset{language=#1}
%     \lstinputlisting[xleftmargin=20pt, label=lst:#3, caption={#4}]{#5}
%     \end{ownfigure}
% }

% % #1 language
% % #2 label
% % #3 caption
% % #4 file
% \newcommand{\lstinput}[4] {
%     \lstinputSeparatedFlag{#1}{#1}{#2}{#3}{#4}
% }

% \newcommand{\lstinputWithoutEnv}[5]{
%     %\stepcounter{table}
%     \vspace{2.5ex}
%     \setlength{\parskip}{1ex plus0pt minus0pt}\noindent%
%     \smash{\rlap{\hspace{0.637ex}\raisebox{-0.2ex}{\rightline{\scriptsize
%     \tt \frame{\makebox(140, 11){#2}}}}}}%
%     \lstset{language=#1}
%     \lstinputlisting[label=lst:#3, caption=#4]{#5}
% }

% Statt Umgebung figure ist jetzt "ownfigure" zu verwenden.
%\renewcommand{\thefigure}{\thetable}
%\AtBeginDocument{%
%\renewcommand{\thelstlisting}{\thetable}
%}%

% Statt Umgebung figure ist jetzt "ownfigure" zu verwenden.
\newenvironment{ownfigure}[0]%
{\begin{figure}[htb!]}%\stepcounter{table}}%
{\end{figure}}

%\newenvironment{ownfigure}[0]%
%{\begin{figure}[htb!]}%\stepcounter{table}}%
%{\end{figure}}

\usepackage{color}
\definecolor{DarkRed}{rgb}{0.75,0,0}
\definecolor{Lightgreen}{rgb}{0.588,1.0,0.588}
\definecolor{DarkGreen}{rgb}{0,0.5,0}
    
\lstdefinelanguage{MontiArc}[]{Java}{
  morekeywords={component, port, in, out, inv, package, import, connect, autoconnect}
}

\lstdefinelanguage{myJava}[]{Java}{
  commentstyle=\color{DarkGreen}\itshape 
}

\lstdefinelanguage{MontiArcAutomaton}[]{Java}{
  morekeywords={component, port, in, out, inv, package, import, connect,
  autoconnect, automaton, state, ocl, java, initial, final,
  noCompletion, chaosCompletion, var, mode, activate, transitions,
  modetransitions}, commentstyle=\color{DarkGreen}\itshape }

%% keywords f�r die MontiCore cfg Dateiern
\lstdefinelanguage{MCConfig} { 
    morekeywords={config, Require, Model} 
}

\lstdefinelanguage{Manifest} { 
    morekeywords={Manifest, Bundle, ManifestVersion, Name, SymbolicName,
      Version, Require
    } 
}

\lstdefinelanguage{mcGrammar}[]{}{
  morekeywords={
    grammar, package, path, parser, lexer, nows, noslcomments, nomlcomments, 
    noident, nostring, noanything, nocharvocabulary, dotident, identrule,
    xmlcomments, hashcomments, texcomments, freemarkercomments, concept, 
    globalnaming, define, usage, options, true, false, protected, ident, 
    compilationunit
  }
}

\lstdefinelanguage{mcLng}[]{}{
  morekeywords={
    dsltool, language, package, path, parser, root, parsingworkflow, 
    rootfactory, lexer, nows, noslcomments, nomlcomments, noident, nostring,
    dotident, concept, globalnaming, define, usage, options, true, false, 
    protected, ident
  }
}

\lstdefinelanguage{mcManifest}[]{}{
  morekeywords={
    bundle, Bundle, Name, SymbolicName, true, false, Main, Class, 
    Version, Activator, Localization, Require, 
    Exclude, Eclipse, LazyStart, Vendor, Export, Package, 
    ClassPath
  }
}

\lstdefinelanguage{Alloy}[]{Java}{
commentstyle=\color{DarkGreen}\itshape,
  morekeywords={abstract,sig,->,fact,pred,fun,run,for,iff,
  not,no,one,all,some,lone,\#,set,in,and,or,but,exactly,none,univ,Int,assert,check},
  otherkeywords = {[2]????},
    morekeywords = {[2]????},
    keywordstyle={[2]\color{blue}},
    otherkeywords = {[3]????,<,<->,->, &, |, =, !=, !,<:,~},
    morekeywords = {[3]????,<,<->,->, &, |, =, !=, !,<:,~},
    keywordstyle={[3]\color{blue}}
  }

\lstdefinelanguage{mccd}[]{Java}{
  morekeywords={classdiagram,abstract,<<singleton>>,class,int,String,
  association,composition,extends}
}

\lstdefinelanguage{FreeMarker}[]{}{
  keywordsprefix={\#},
  keywords={in},
  commentstyle=\color{DarkGreen}\itshape }


\lstdefinelanguage{Mona}[]{}{
  morekeywords={ex0,all0,ex1,all1,ex2,all2,var0,var1,var2,pred,in,notin,include,union,inter,empty,assert},
  morecomment=[l]{\#},
  commentstyle=\color{DarkGreen}\itshape,
  otherkeywords = {[2]????,next,boolean,init,case,esac},
  morekeywords = {[2]????,next,boolean,init,case,esac},
  otherkeywords = {[3]????,<,<=>,=>, &, |, =, !=, !},
  morekeywords = {[3]????,<,<=>,=>, &, |, =, !=, !},
}

\lstdefinelanguage{myPython}[]{Python}{
  morekeywords={assert},
  morecomment=[l]{\#},
  commentstyle=\color{DarkGreen}\itshape,
}

\lstdefinelanguage{GeneratorConfiguration}[]{Java} {
  morekeywords={
    template, 
    generator, 
    ast, 
    runtime},
}

\lstdefinelanguage{ApplicationConfiguration}[]{Java} {
  morekeywords={
    application,
    behaviors,
    bindings,
    classdiagrams,
    components,
    factories,
    generators,
    map,
    to},
}

\lstdefinelanguage{Isabelle}[]{} {
    morekeywords={
        datatype,
        typedef},
}
